DINAMITE: A modern approach to memory performance profiling

Diagnosing and fixing performance problems on multicore machines with deep memory hierarchies is extremely challenging. Certain problems are best addressed when we can analyze the entire trace of program execution, e.g., every memory access. Unfortunately such detailed execution logs are very large and cannot be analyzed by direct inspection. We present DINAMITE: a toolkit for Dynamic INstrumentation and Analysis for MassIve Trace Exploration. DINAMITE is a collection of tools for end-to-end performance analysis: from the LLVM compiler pass that instruments the program to plug-and-play tools that use a modern data analytics engine Spark Streaming for trace introspection. Using DINAMITE we found opportunities to improve data layout in several applications that resulted in 15-20% performance improvements and found a shared-variable bottleneck in a popular key-value store, whose elimination improved performance by 20x.

==> conclusion.tex <==
%auto-ignore
\section{Conclusion}\label{sec:conclusion}

